Saving Critical Nodes with Firefighters is FPT

We consider the problem of firefighting to save a critical subset of nodes. The firefighting game is a turn-based game played on a graph, where the fire spreads to vertices in a breadth-first manner from a source, and firefighters can be placed on yet unburnt vertices on alternate rounds to block the fire. In this work, we consider the problem of saving a critical subset of nodes from catching fire, given a total budget on the number of firefighters. We show that the problem is para-NP-hard when parameterized by the size of the critical set. We also show that it is fixed-parameter tractable on general graphs when parameterized by the number of firefighters. We also demonstrate improved running times on trees and establish that the problem is unlikely to admit a polynomial kernelization (even when restricted to trees). Our work is the first to exploit the connection between the firefighting problem and the notions of important separators and tight separator sequences. Finally, we consider the spreading model of the firefighting game, a closely related problem, and show that the problem of saving a critical set parameterized by the number of firefighters is W[2]-hard, which contrasts our FPT result for the non-spreading model.

==> ffcs-pre.tex <==
In this section, we introduce the notation and the terminology that we will need to describe our algorithms. Most of our notation is standard. We use $[k]$ to denote the set $\{1,2,\ldots,k\}$, and we use $[k]_\OO$ and $[k]_\EE$, respectively, to denote the odd and even numbers in the set $[k]$.

\subparagraph*{Graphs, Important Separators and Tight Separator Sequences.} We introduce here the most relevant definitions, and use standard notation pertaining to graph theory based on~\cite{PCBook-CyganEtAl,Diestel:2012vm}. All our graphs will be simple and undirected unless mentioned otherwise. For a graph $G = (V,E)$ and a vertex $v$, we use $N(v)$ and $N[v]$ to refer to the open and closed neighborhoods of $v$, respectively. The \emph{distance} between vertices $u,v$ of $G$ is the length of a shortest path from $u$ to $v$ in $G$; if no such path exists, the distance is defined to be $\infty$. A graph $G$ is said to be \emph{connected} if there is a path in $G$ from every vertex of $G$ to every other vertex of $G$. If $U\subseteq V$ and $G\left[U\right]$ is connected, then $U$ itself is said to be connected in $G$.  For a subset $S \subseteq V$, we use the notation $G\setminus S$ to refer to the graph induced by the vertex set $V \setminus S$. 

The following definitions about important separators and tight separator sequences will be relevant to our main \FPT{} algorithm. We first define the notion of the reachability set of a subset $X$ with respect to a subset $S$. 

\begin{definition}[Reachable Sets \cite{}]
	Let $G = (V, E)$ be an undirected graph, let $X \subseteq V$ and $S \subseteq V \setminus X$. We denote by $R_G(X,S)$ the set of vertices of $G$ \textit{reachable} from $X$ in $G \setminus S$ and by $NR_G(X, S)$ the set of vertices of $G$ not reachable from $X$ in $G \setminus S$. We drop the subscript $G$ if it is clear from the context.
\end{definition}

We now turn to the notion of an $X$-$Y$ separator and what it means for one separator to cover another. 

\begin{definition}[Covering by Separators \cite{}]
	Let $G = (V, E)$ be an undirected graph and let $X, Y \subset V$ be two disjoint vertex sets. A subset $S \subseteq V \setminus (X \cup Y )$ is called an $X-Y$ separator in $G$ if $R_G(X, S) \cap Y = \emptyset$, or in other words, there is no path from $X$ to $Y$ in the graph $G \setminus S$. We denote by $\lambda_G (X, Y)$ the size of the smallest $X-Y$ separator in $G$. An $X-Y$ separator $S_1$ is said to \textit{cover} an $X-Y$ separator $S$ with respect to $X$ if $R(X,S_1) \supset R(X,S)$. If the set $X$ is clear from the context, we just say that $S_1$ covers $S$. An $X-Y$ separator is said to be inclusionwise minimal if none of its proper subsets is an $X-Y$ separator.
\end{definition}

If $X = \{x\}$ is a singleton, then we abuse notation and refer to a $x-Y$ separator rather than a $\{x\}-Y$ separator. A separator $S_1$ dominates $S$ if it covers $S$ and is not larger than $S$ in size:

\begin{definition}[Dominating Separators \cite{}]
	Let $G = (V, E)$ be an undirected graph and let $X, Y \subset V$ be two disjoint vertex sets. An $X-Y$ separator $S_1$ is said to \textit{dominate} an $X-Y$ separator $S$ with respect to $X$ if $|S_1| \leq |S|$ and $S_1$ covers $S$ with respect to $X$. If the set $X$ is clear from the context, we just say that $S_1$ dominates $S$.
\end{definition}

We finally arrive at the notion of important separators, which are those that are not dominated by any other separator.

\begin{definition}[Important Separators \cite{}] Let $G = (V, E)$ be an undirected graph, $X, Y \subset V$ be disjoint vertex sets and $S \subseteq V \setminus (X \cup Y)$ be an $X-Y$ separator in $G$. We say that $S$ is an \textit{important} $X-Y$ separator if it is inclusionwise minimal and there does not exist another $X-Y$ separator $S_1$ such that $S_1$ dominates $S$ with respect to $X$. \end{definition}

It is well known that the important separator of smallest size is, in fact, unique:

\begin{lemma} \cite{}
	Let $G = (V, E)$ be an undirected graph, $X, Y \subset V$ be disjoint vertex sets. There exists a unique important $X-Y$ separator $S^\star$ of size $\lambda_G(X,Y)$.
\end{lemma}

It is also useful to know that the number of important separators is bounded as an \FPT{} function of the size of the important separators. 

\begin{lemma} \cite{} Let $G = (V, E)$ be an undirected graph, $X, Y \subset V$ be disjoint vertex sets of $G$. For every $k \geq 0$ there are at most $4^k$ important $X-Y$ separators of size at most $k$. Furthermore, there is an algorithm that runs in time $4^kk(m + n)$ which enumerates all such important X-Y separators, where $n = |V|$ and $m = |E|$.
\end{lemma}

We are now ready to define tight separator sequences.


\begin{definition}[Important Separators of Order $i$\cite{}]
\label{def:tss}
Let $G = (V, E)$ be a graph and let $X, Y \subseteq V$ be disjoint vertex sets. We define an important $X,Y$-separator of order $i$, $S^i$, to be the unique smallest important $X-S^{i-1}$-separator in $G$, where $S^0 = Y$.
\end{definition}

\begin{definition}[Tight Separator Sequences \cite{}] Let $G = (V,E)$ be a graph and let $X, Y \subseteq V$. Let $\ell \geq 1$ be such that there is no important $X-Y$ separator of order $\ell+1$. We define a tight $X-Y$ separator sequence $I$ to be a set $I = \{S^i |1 \leq i \leq \ell \}$, where $S^i$ is an important $X-Y$ separator of order $i$.
\end{definition}

It turns out that tight separator sequences are unique, and can also be computed in polynomial time~\cite{}.

\begin{lemma}[\cite{}]
Let $G = (V, E)$ be a graph and let $X, Y \subseteq V$. A tight $X-Y$ separator sequence is unique and can be computed in polynomial time.
\end{lemma} 

\subparagraph{Saving a Critical Set.} We now turn to the definition of the firefighting problem. The game proceeds as described earlier: we are given a graph $G$ with a vertex $s \in V(G)$. To begin with, the fire breaks out at $s$ and vertex $s$ is burning. At each step $t \geq 1$, first the firefighter protects one vertex not yet on fire - this vertex remains permanently protected - and the fire then spreads from burning vertices to all unprotected neighbors of these vertices. The process stops when the fire cannot spread anymore. In the definitions that follow, we formally define the notion of a firefighting strategy. 

\begin{definition}[Firefighting Strategy] A $k$-step firefighting strategy is defined as a function $\mathfrak{h}: [2k]_{\OO} \rightarrow V(G)$. 	Such a strategy is said to be \textit{valid in $G$ with respect to $s$} if, for all $i \in [kk]_{\OO}$, when the fire breaks out in $s$ and firefighters are placed according to $\mathfrak{h}$ for all time steps up to $i-2$, the vertex $\mathfrak{h}(i)$ is not burning at time step $i$. If $G$ and $s$ are clear from the context, we simply say that $\mathfrak{h}$ is a valid strategy.
\end{definition}

\begin{definition}[Saving $C$] For a vertex $s$ and a subset $C \subseteq V(G) \setminus \{s\}$, a firefighting strategy $\mathfrak{h}$ is said to save $C$ if $\mathfrak{h}$ is a valid strategy and $\{\mathfrak{h}(i)~|~ i \in [kk]_{\OO} \}$ is a $\{s\}$-$C$ separator in $G$, in other words, there is no path from $s$ to any vertex in $C$ if firefighters are placed according to $\mathfrak{h}$.	
\end{definition}

We are now ready to define the parameterized problem that is the focus of this work.

\problembox{\sacs{}~(\SACS{})}{An undirected $n$-vertex graph $G$, a vertex $s$, a subset $C \subseteq V(G) \setminus \{s\}$, and an integer k.}{$k$}{Is there a valid $k$-step strategy that saves $C$ when a fire breaks out at $s$?}

\nmtodo{Need to define the spreading model and the $b$-firefighters-per-step model here as well, assuming we go in that direction.}



\subparagraph*{Parameterized Complexity.} We follow standard terminology pertaining to parameterized algorithms based on the monograph~\cite{PCBook-CyganEtAl}. Here we define a known technique to prove kernel lower bounds, called cross composition. Towards this, we first define polynomial equivalence relations. 

\begin{definition}[polynomial equivalence relation~\cite{BJK11}] \label{polyEquivalenceRelation}
An equivalence relation~${\cal R}$ on~$\Sigma^*$, where $\Sigma$ is a finite alphabet, is called a \emph{polynomial equivalence relation} if the following holds:
%\begin{enumerate}
%	\item 
$(1)$ equivalence of any~$x,y \in \Sigma^*$ can be checked in time polynomial in~$|x|+|y|$, %There is an algorithm that given two strings~$x,y \in \Sigma^*$ decides whether~$x$ and~$y$ belong to the same equivalence class in~$(|x| + |y|)^{\Oh(1)}$ time.
 and $(2)$	any finite set~$S \subseteq \Sigma^*$ has at most~$(\max _{x \in S} |x|)^{O(1)}$~equivalence classes.
%\end{enumerate}
\end{definition}


\begin{definition}[cross-composition~\cite{BJK11}] \label{crossComposition}
Let~$L \subseteq \Sigma^*$ and let~$Q \subseteq \Sigma^* \times \mathbb{N}$ be a parameterized problem. We say that~$L$ \emph{cross-composes} into~$Q$ if there is a polynomial equivalence relation~${\cal R}$ and an algorithm which, given~$t$ strings~$x_1, x_2, \ldots, x_t$ belonging to the same equivalence class of~${\cal R}$, computes an instance~$(x^*,k^*) \in \Sigma^* \times \mathbb{N}$ in time polynomial in~$\sum _{i=1}^t |x_i|$ such that: (i) $(x^*, k^*) \in Q \Leftrightarrow x_i \in L$ for some $1 \leq i \leq t$  and (ii) $k^*$ is bounded by a polynomial in ($\max _{1\leq i\leq t} |x_i|+\log t$).
\end{definition}

The following theorem allows us to rule out the existence of a polynomial kernel for a parameterized problem.

\begin{theorem}[\cite{BJK11}]%[\nothere{}]
\label{theorem:conp:crosscomposition}
If an \NPH problem~$L\subseteq \Sigma^*$ has a cross-composition into the parameterized problem~$Q$ and~$Q$ has a polynomial kernel then NP $\subseteq$ coNP/poly.
\end{theorem}



%\problembox{\name{Critical Vertex Firefighting}}{An undirected $n$-vertex graph $G$, vertices $s,t$, and an integer k.}{$k$}{Is there a $k$-step strategy that saves $t$ when a fire breaks out at $s$?}

==> ffcs-prelims-formatted.tex <==
We use standard notation pertaining to Graph Theory and Parameterized Algorithms, based on the books~\cite{}.[1]

\problembox{\name{Critical Vertex Firefighting}}{An undirected $n$-vertex graph $G$, vertices $s,t$, and an integer k.}{$k$}{Is there a strategy that saves $t$ when a fire breaks out at $s$?}

\problembox{\name{Critical Set Firefighting}}{An undirected $n$-vertex graph $G$, a vertex $s$, a subset $T \subseteq V(G) \setminus \{s\}$, and an integer k.}{$k$}{Is there a strategy that saves $t$ when a fire breaks out at $s$?}
[1]	R. Diestel, Graph Theory. Reinhard Diestel, 2012.

